Adaptive Uncertainty Quantification for Generative AI

This work is concerned with conformal prediction in contemporary applications (including generative AI) where a black-box model has been trained on data that are not accessible to the user. Mirroring split-conformal inference, we design a wrapper around a black-box algorithm which calibrates conformity scores. This calibration is local and proceeds in two stages by first adaptively partitioning the predictor space into groups and then calibrating sectionally group by group. Adaptive partitioning (self-grouping) is achieved by fitting a robust regression tree to the conformity scores on the calibration set. This new tree variant is designed in such a way that adding a single new observation does not change the tree fit with overwhelmingly large probability. This add-one-in robustness property allows us to conclude a finite sample group-conditional coverage guarantee, a refinement of the marginal guarantee. In addition, unlike traditional split-conformal inference, adaptive splitting and within-group calibration yields adaptive bands which can stretch and shrink locally. We demonstrate benefits of local tightening on several simulated as well as real examples using non-parametric regression. Finally, we consider two contemporary classification applications for obtaining uncertainty quantification around GPT-4o predictions. We conformalize skin disease diagnoses based on self-reported symptoms as well as predicted states of U.S. legislators based on summaries of their ideology. We demonstrate substantial local tightening of the uncertainty sets while attaining similar marginal coverage.

==> todo-list.tex <==


12:00 pm Friday C-09 Veronika's AI talk
1: oo pm Friday Conformal meeting at V's office


1. [X] Modify tables to add optimal m and K values: show n in the left column
Add (m,K) inside the table for our method only, not for all the other methods!
Make tree table, and forest table separate, instead of ISL table and PB Table
Include conformal forest

2. [X] Make a second version where the calibration size is limited to maybe 500 for each dataset.

3. Elaborate on the benefit of interpretability for the groups that is gained by the dyadic tree - In the section when we are discussing the table, we can add a reference to the later tree plots that are used for interpretability

4. [X] Above section 4.2, re-populate with the new values for the ten random trials!

5. For Figure 12,13 - remake it with the new trees

6. [X] Rewrite Section C - sensitivity analysis, based on the new validation heatmaps

7. [X] Merge figure 8 and 9 into side-by-side

8. [X] Remove Table 2

9. [X] Use s1-large, s2-large, not s1 and s2

